Meson correlators in the epsilon-regime of two-flavor lattice QCD

We calculate the meson correlators in the $\epsilon$-regime of two-flavor QCD. On a $16^3\times 32$ lattice with $a\sim 0.11$ fm, the lattice simulations are performed with the dynamical overlap fermions. We reduce the sea quark mass down to $\sim$ 3 MeV and the valence quark masses are taken in the range 1-4 MeV. The meson correlators in various channels are compared with the predictions of (partially quenched) chiral perturbation theory (ChPT). Including the NLO order of the $\epsilon$-expansion, we extract the leading-order low energy constants of ChPT, the pion decay constant $F$ and the chiral condensate $\Sigma$, as $F=87.3(5.5)$ MeV and $\Sigma^{\bar{\mathrm{MS}}}=[237.8(4.0){MeV}]^3$.

==> sec5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% section conclusion %%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We performed the QCD simulation with two dynamical
quarks of which Dirac operator has an exact chiral symmetry.
The sea quark mass achieved the almost physical value
around 3 MeV, which is light enough to reach the 
$\epsilon$-regime of QCD with the lattice size
around $L\sim 1.7$ fm.
We measured the various channels of meson correlators
in $\nu=0$ topological sector,
with 4 different valence quark masses 
from $\sim$ 1 MeV to $\sim$ 4 MeV.

In the degenerate case $m_v=m_s=0.002$,
from the axial-vector correlator which is sensitive to
the pion decay constant $F$, and the pseudo-scalar 
correlator which is sensitive to 
the chiral condensate $\Sigma$,
we determine the low-energy constant of ChPT:
%\begin{eqnarray}
$\Sigma^{\overline{\mathrm{MS}}}(\mathrm{2~GeV}) = [239.8(4.0)\mbox{~MeV}]^3$
and 
  %&\mbox{and}& 
$F_\pi = 87.3(5.6) [\sqrt{2}F_\pi = 123.5(7.9)]\mbox{MeV}$,
%\end{eqnarray}
to ${\cal O}(\epsilon^2)$ order.

The values are compared with ChPT predictions in
the other channels (scalar and vector),
with the different valence quark masses, 
and the result from the Dirac spectrum in our previous work.
All of them are consistent with each other, 
within the statistical errors.
They are insensitive to the fitting range if we take the
nearest fitting point larger than $\sim 1.1$fm.

Thus, we could measure the low-energy constant with a higher
accuracy $\sim O(\epsilon^2)$ than that of our previous work.
The discrepancy of $F$ from the $p$-regime result, 
however, suggests some unexpectedly 
large $O(\epsilon^4)\sim 1/V$ error and so on.
In fact, $O(\epsilon^2)\sim 1/V^{1/2}$ is already considerably large,
$\sim 10$\%.
Further studies, with larger volume, are important
to confirm our results.

